SnapNTell: Enhancing Entity-Centric Visual Question Answering with Retrieval Augmented Multimodal LLM

Vision-extended LLMs have made significant strides in Visual Question Answering (VQA). Despite these advancements, VLLMs still encounter substantial difficulties in handling queries involving long-tail entities, with a tendency to produce erroneous or hallucinated responses. In this work, we introduce a novel evaluative benchmark named \textbf{SnapNTell}, specifically tailored for entity-centric VQA. This task aims to test the models' capabilities in identifying entities and providing detailed, entity-specific knowledge. We have developed the \textbf{SnapNTell Dataset}, distinct from traditional VQA datasets: (1) It encompasses a wide range of categorized entities, each represented by images and explicitly named in the answers; (2) It features QA pairs that require extensive knowledge for accurate responses. The dataset is organized into 22 major categories, containing 7,568 unique entities in total. For each entity, we curated 10 illustrative images and crafted 10 knowledge-intensive QA pairs. To address this novel task, we devised a scalable, efficient, and transparent retrieval-augmented multimodal LLM. Our approach markedly outperforms existing methods on the SnapNTell dataset, achieving a 66.5\% improvement in the BELURT score. We will soon make the dataset and the source code publicly accessible.

==> checklist.tex <==


% Enviroment for numbered tabular
\newenvironment{enumtabular}[2]
 {%
  \setcounter{myenumi}{0}%
  \setcounter{myenumii}{0}%
  \renewcommand{\item}{#1\refstepcounter{myenumi}\themyenumi.\ \  }%
  \begin{longtable}{#2}
 }
 {\end{longtable}}


% Command for choice menu 
\newcommand{\cm}[3]{\mbox{\ChoiceMenu[height=0.3cm,width=0.3cm,bordercolor=,name=#1,radio,radiosymbol=\ding{108},default=#3]{}{#2}}}

% Command for text field
\newcommand{\tf}[3][0.78]{\mbox{\TextField[bordercolor=,name=#2,value={#3},multiline=true,height=4em, width=#1\textwidth]{\noindent \parbox{0.11\textwidth}{Section or\\Justification}}}}

% Command for checkbox
\newcommand{\cb}[1]{\mbox{\CheckBox[bordercolor=,name=#1,height=0.4cm,width=0.4cm]{}{\ }}}

% Fix choice menu
\makeatletter
    \patchcmd{\HyField@FlagsRadioButton}{\HyField@SetFlag{Ff}{Radio}}{}{}{}
\makeatother

\titleformat{\section}{\Large\bfseries}{\Alph{section}}{1em}{}
\titleformat{\subsection}{\normalfont\bfseries}{\Alph{section}\arabic{subsection}}{1em}{}

\title{Responsible NLP Research Checklist\vspace{-3em}}
\date{}

\begin{document}
\maketitle

Members of the ACL are responsible for adhering to the \href{https://www.aclweb.org/portal/content/acl-code-ethics}{ACL code of ethics}. The ARR Responsible NLP Research checklist is designed to encourage best practices for responsible research, addressing issues of research ethics, societal impact and reproducibility.

Please read the \href{https://aclrollingreview.org/responsibleNLPresearch/}{Responsible NLP Research checklist guidelines} for information on how to answer these questions. Note that not answering positively to a question is not grounds for rejection. 

All supporting evidence can appear either in the main paper or the supplemental material. For each question, if you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification.

Please do \textbf{not} modify, reorder, delete or add questions, question options or other wording of this document.

% USAGE:
% Use the last argument in the \cm and \tf commands to mark your answer, e.g.:
% \cm{mainClaims}{Yes,No,N/A}{N/A}
% \tf[0.85]{mainClaimsJustification}{This does not apply...}

\section{For every submission}

\subsection{Did you discuss the \textit{limitations} of your work?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{mainClaims}{Yes}{}\\[0.2cm]
    \tf[0.85]{mainClaimsJustification}{Limitations section on Page 9.}
\end{tabular}
\end{Form} \\[0.3cm]
        
\subsection{Did you discuss any potential \textit{risks} of your work?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{risks}{N/A}{}\\[0.2cm]
    \tf[0.85]{risksJustification}{Ethics Statement and Broader Impact sections on Page 9.}
\end{tabular}
\end{Form}

\subsection{Do the abstract and introduction summarize the paper’s main claims?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{abstractIntro}{Yes}{}\\[0.2cm]
    \tf[0.85]{abstractIntroJustification}{We provided the summary of this work in the abstract and introduction (Section 1). }
\end{tabular}
\end{Form}

\section{Did you use or create \textit{scientific artifacts}?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, you can skip the rest of this section. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
\cm{createArtifacts}{Yes}{}\\[0.2cm]
\tf{citeCreatorsJustification}{Section 3.}
\end{tabular}
\end{Form}

If yes:
\subsection{Did you cite the creators of artifacts you used?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
   \begin{tabular}{l}
    \cm{citeCreators}{Yes}{}\\[0.2cm]
    \tf{citeCreatorsJustification}{Section 3.}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss the \textit{license or terms} for use and/or distribution of any artifacts?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
   \begin{tabular}{l}
    \cm{legalGrounds}{Yes}{}\\[0.2cm]
    \tf{legalGroundsJustification}{In abstract (``We will soon make the dataset
029 and the source code publicly accessible") and Section 3.}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss if your use of existing artifact(s) was consistent with their \textit{intended use}, provided that it was specified? For the artifacts you create, do you specify intended use and whether that is compatible with the original access conditions (in particular, derivatives of data accessed for research purposes should not be used outside of research contexts)?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
   \begin{tabular}{l}
    \cm{intendedUse}{Yes}{}\\[0.2cm]
    \tf{intendedUseJustification}{In abstract (``We will soon make the dataset
029 and the source code publicly accessible") and Sections 3 \& 5.}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss the steps taken to check whether the data that was collected/used contains any \textit{information that names or uniquely identifies individual people} or \textit{offensive content}, and the steps taken to protect / anonymize it?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{personallyIdentifiableInformationOrOffensiveContent}{N/A}{}\\[0.2cm]
    \tf{personallyIdentifiableInformationOrOffensiveContentJustification}{Sections 3.}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you provide documentation of the artifacts, e.g., coverage of domains, languages, and linguistic phenomena, demographic groups represented, etc.?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{documentation}{Yes}{}\\[0.2cm]
    \tf{documentationJustification}{Sections 3 and Appendix A,B,C,D.}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you report relevant statistics like the number of examples, details of train/test/dev splits, etc. for the data that you used/created?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{relevantStatistics}{Yes}{}\\[0.2cm]
    \tf{relevantStatisticsJustification}{Sections 3 and Appendix A,B,C,D.}
\end{tabular}
\end{Form} \\[0.3cm]

\section{Did you run \textit{computational experiments}?} 
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, you can skip the rest of this section. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{computationalExperiments}{Yes}{Section 4}
\end{tabular}
\end{Form}

If yes:
\subsection{Did you report the \textit{number of parameters} in the models used, the \textit{total computational budget} (e.g., GPU hours), and \textit{computing infrastructure} used?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{reportReproducibility}{Yes}{}\\[0.2cm]
    \tf{reportReproducibilityJustification}{Section 5.}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss the experimental setup, including \textit{hyperparameter search} and \textit{best-found hyperparameter} values?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{bestFoundHyperparameter}{Yes}{}\\[0.2cm]
    \tf{bestFoundHyperparameterJustification}{Section 5.}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you report \textit{descriptive statistics} about your results (e.g., error bars around results, summary statistics from sets of experiments), and is it transparent whether you are reporting the max, mean, etc. or just a single run?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{descriptiveStatistics}{Yes}{}\\[0.2cm]
    \tf{descriptiveStatisticsJustification}{Section 5.}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{If you used existing packages (e.g., for preprocessing, for normalization, or for evaluation), did you report the implementation, model, and parameter settings used (e.g., NLTK, Spacy, ROUGE, etc.)?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{existingPackages}{Yes}{}\\[0.2cm]
    \tf{existingPackagesJustification}{Section 5.}
\end{tabular}
\end{Form} \\[0.3cm]

\section{Did you use \textit{human annotators} (e.g., crowdworkers) or \textit{research with human subjects}?}  If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, you can skip the rest of this section. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{hummanAnnotators}{Yes}{}\\[0.2cm]
    \tf{existingPackagesJustification}{Section 3.}
\end{tabular}
\end{Form}

If yes:
\subsection{Did you report the full text of instructions given to participants, including e.g., screenshots, disclaimers of any risks to participants or annotators, etc.?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{fullTextInstructions}{Yes}{}\\[0.2cm]
    \tf{fullTextInstructionsJustification}{Section 3.}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you report information about how you recruited (e.g., crowdsourcing platform, students) and paid participants, and discuss if such \textit{payment is adequate} given the participants’ demographic (e.g., country of residence)?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{payment}{Yes}{}\\[0.2cm]
    \tf{paymentJustification}{Section 3.}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss whether and how \textit{consent} was obtained from people whose data you're using/curating (e.g., did your instructions explain how the data would be used)?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{consent}{Yes}{}\\[0.2cm]
    \tf{consentJustification}{Section 3.}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Was the data collection protocol \textit{approved (or determined exempt)} by an ethics review board?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{ethicsAmountSpent}{Yes}{}\\[0.2cm]
    \tf{ethicsAmountSpentJustification}{Section 3.}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you report the basic demographic and geographic characteristics of the \textit{annotator} population that is the source of the data?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{annotator}{Yes}{}\\[0.2cm]
    \tf{annotatorJustification}{Section 3.}
\end{tabular}
\end{Form} 


==> tables/blip.tex <==
\begin{tabular}{lrrrrrrrrrr}\toprule
Method &ROUGE-1 &ROUGE-2 &ROUGE-L &BLEU-1 &BLEU-2 &BLEU-3 &BLEU-4 &METEOR &BertScore \\
\midrule
landmark &17.21 &6.02 &15.71 &2.57 &0.91 &0.37 &0.22 &7.79 &82.70 \\
painting &17.74 &5.55 &15.99 &4.64 &1.70 &0.50 &0.18 &9.60 &83.25 \\
sculpture &15.65 &5.17 &14.00 &2.07 &0.53 &0.18 &0.01 &6.34 &82.90 \\
food &18.40 &4.11 &16.70 &3.30 &1.12 &0.31 &0.04 &7.19 &83.54 \\
fruit &12.77 &4.23 &11.93 &4.45 &2.38 &1.45 &0.94 &7.08 &81.27 \\
vegetable &15.11 &4.93 &14.20 &4.92 &2.37 &1.11 &0.81 &8.72 &82.20 \\
mammal &15.80 &4.91 &14.63 &4.34 &1.83 &0.77 &0.40 &8.21 &82.43 \\
amphibian &13.90 &3.54 &12.87 &3.29 &1.41 &0.78 &0.52 &7.13 &81.75 \\
insect &13.42 &4.28 &11.95 &4.86 &2.64 &0.96 &0.57 &7.45 &82.30 \\
fish &12.53 &3.33 &11.53 &3.96 &1.69 &0.81 &0.53 &6.61 &81.45 \\
bird &11.86 &2.53 &10.92 &2.01 &0.59 &0.25 &0.12 &5.30 &81.66 \\
reptile &14.80 &3.96 &13.81 &4.34 &2.17 &1.28 &0.64 &7.94 &82.57 \\
celebrity &9.07 &2.70 &8.40 &1.90 &0.79 &0.41 &0.23 &4.39 &81.33 \\
instrument &16.81 &5.46 &15.55 &4.44 &2.37 &1.43 &0.70 &8.51 &83.23 \\
plant &11.32 &2.57 &10.66 &2.99 &1.12 &0.50 &0.37 &5.58 &80.60 \\
electronics &23.10 &9.16 &20.90 &8.01 &4.91 &2.82 &1.49 &12.61 &85.74 \\
tool &23.23 &9.57 &21.09 &8.29 &4.65 &2.46 &1.16 &13.07 &85.52 \\
transportation &20.61 &7.92 &19.38 &7.60 &4.25 &1.32 &0.63 &11.79 &85.03 \\
sport &16.59 &5.63 &14.99 &4.67 &2.07 &1.15 &0.65 &8.70 &83.43 \\
book &15.35 &6.41 &14.34 &3.14 &1.00 &0.24 &0.17 &8.53 &82.53 \\
household &23.37 &9.72 &21.26 &7.42 &3.97 &1.54 &1.01 &12.84 &85.35 \\
car &19.67 &8.03 &19.16 &3.60 &1.45 &0.58 &0.15 &11.43 &83.62 \\
\bottomrule
\end{tabular}

==> tables/instructblip.tex <==
\begin{tabular}{lrrrrrrrrrr}\toprule
Method &ROUGE-1 &ROUGE-2 &ROUGE-L &BLEU-1 &BLEU-2 &BLEU-3 &BLEU-4 &METEOR &BertScore \\
\midrule
landmark &13.49 &5.00 &11.56 &5.50 &3.42 &1.96 &1.22 &8.55 &77.46 \\
painting &11.40 &3.94 &10.24 &4.11 &1.91 &1.17 &0.87 &7.01 &78.73 \\
sculpture &11.68 &2.89 &9.96 &3.78 &2.20 &1.39 &0.74 &6.38 &78.34 \\
food &14.25 &4.30 &12.68 &4.13 &2.27 &1.32 &0.61 &7.83 &74.05 \\
fruit &11.23 &3.61 &10.39 &3.84 &2.35 &1.33 &1.22 &6.10 &65.29 \\
vegetable &12.55 &5.17 &11.46 &4.88 &2.83 &1.62 &1.33 &8.69 &67.82 \\
mammal &10.42 &3.31 &9.48 &3.97 &2.17 &1.29 &0.91 &6.10 &72.33 \\
amphibian &10.48 &3.71 &9.36 &3.25 &2.37 &1.48 &1.04 &7.41 &79.90 \\
insect &8.33 &2.95 &7.81 &3.57 &2.20 &1.41 &0.77 &5.92 &64.89 \\
fish &9.52 &3.59 &8.78 &3.81 &2.34 &1.65 &1.15 &6.30 &62.66 \\
bird &8.81 &2.53 &8.10 &2.81 &1.50 &0.38 &0.24 &5.09 &73.04 \\
reptile &14.05 &5.47 &12.59 &5.58 &3.66 &1.88 &1.32 &9.54 &73.28 \\
celebrity &5.39 &1.43 &5.01 &1.10 &0.56 &0.24 &0.10 &2.82 &78.22 \\
instrument &13.95 &5.43 &12.05 &6.85 &4.64 &2.97 &2.03 &9.16 &79.52 \\
plant &9.89 &2.61 &9.29 &2.43 &0.74 &0.45 &0.35 &5.05 &76.41 \\
electronics &14.98 &5.43 &12.87 &5.92 &3.46 &1.93 &1.09 &10.31 &75.86 \\
tool &13.83 &4.46 &12.35 &5.87 &3.35 &1.96 &1.39 &9.37 &71.88 \\
transportation &13.22 &4.29 &11.47 &5.68 &3.10 &1.69 &1.03 &9.60 &79.65 \\
sport &13.00 &3.80 &10.89 &5.33 &2.78 &1.32 &0.55 &8.96 &79.67 \\
book &12.10 &6.84 &11.50 &4.83 &3.34 &2.42 &1.37 &8.31 &76.68 \\
household &16.98 &7.32 &15.15 &5.92 &3.51 &1.82 &1.07 &11.73 &79.17 \\
car &14.14 &3.05 &12.87 &4.57 &2.57 &0.71 &0.48 &6.78 &82.32 \\
\bottomrule
\end{tabular}

==> tables/llava.tex <==
\begin{tabular}{lrrrrrrrrrr}\toprule
Method &ROUGE-1 &ROUGE-2 &ROUGE-L &BLEU-1 &BLEU-2 &BLEU-3 &BLEU-4 &METEOR &BertScore \\
\midrule
landmark &33.98 &15.15 &27.57 &22.10 &13.06 &8.20 &4.68 &25.79 &86.61 \\
painting &30.59 &13.89 &25.49 &20.76 &12.51 &7.96 &4.79 &25.37 &86.63 \\
sculpture &38.93 &19.64 &32.21 &25.28 &16.82 &11.23 &7.95 &29.58 &87.69 \\
food &28.45 &10.58 &22.66 &16.31 &8.79 &4.36 &2.41 &23.34 &86.88 \\
fruit &36.12 &21.51 &33.41 &24.84 &18.44 &14.13 &11.67 &30.98 &87.25 \\
vegetable &32.92 &17.60 &28.63 &21.18 &14.74 &10.55 &8.56 &28.56 &86.91 \\
mammal &30.37 &12.29 &25.10 &19.15 &10.77 &5.87 &4.02 &24.02 &86.57 \\
amphibian &29.06 &13.26 &24.89 &18.99 &12.45 &8.25 &6.29 &25.18 &86.33 \\
insect &30.61 &15.74 &25.54 &19.27 &13.25 &9.30 &6.70 &29.23 &86.82 \\
fish &35.02 &19.26 &30.76 &23.97 &17.01 &12.71 &10.15 &30.25 &87.05 \\
bird &32.97 &16.34 &28.93 &23.02 &15.61 &10.89 &8.66 &26.82 &86.51 \\
reptile &36.20 &20.22 &32.53 &24.74 &17.80 &12.72 &10.55 &30.39 &87.77 \\
celebrity &26.80 &12.85 &22.66 &17.89 &11.19 &7.16 &3.50 &19.37 &85.90 \\
instrument &32.06 &12.87 &25.90 &20.28 &11.90 &6.79 &4.42 &26.34 &87.24 \\
plant &35.43 &18.84 &30.10 &24.62 &16.87 &10.70 &8.52 &28.76 &86.40 \\
electronics &28.35 &12.15 &22.19 &16.65 &9.94 &6.27 &3.88 &28.50 &87.38 \\
tool &27.46 &11.78 &21.69 &16.73 &9.99 &6.32 &3.88 &27.99 &87.29 \\
transportation &27.39 &12.42 &22.13 &16.20 &9.99 &6.53 &4.45 &27.91 &87.47 \\
sport &25.31 &8.90 &19.23 &14.90 &7.64 &3.73 &1.79 &23.05 &86.23 \\
book &31.77 &15.62 &27.70 &21.04 &12.40 &8.14 &5.25 &25.29 &86.21 \\
household &30.39 &13.94 &24.28 &17.77 &11.17 &7.35 &4.95 &27.99 &87.74 \\
car &42.28 &19.03 &37.35 &28.36 &18.04 &8.03 &5.63 &28.58 &88.51 \\
\bottomrule
\end{tabular}

==> tables/minigpt4.tex <==
\begin{tabular}{lrrrrrrrrrr}\toprule
Method &ROUGE-1 &ROUGE-2 &ROUGE-L &BLEU-1 &BLEU-2 &BLEU-3 &BLEU-4 &METEOR &BertScore \\
\midrule
landmark &30.91 &12.95 &25.11 &20.03 &11.56 &7.13 &4.28 &24.11 &86.31 \\
painting &27.61 &11.60 &23.50 &18.13 &10.18 &6.67 &4.13 &22.14 &86.27 \\
sculpture &35.13 &16.53 &29.67 &23.44 &15.10 &9.88 &6.29 &27.33 &87.24 \\
food &30.40 &11.02 &25.14 &17.45 &8.68 &4.78 &2.47 &21.54 &87.20 \\
fruit &34.86 &20.99 &32.42 &24.33 &18.06 &14.55 &11.90 &29.66 &87.01 \\
vegetable &29.61 &15.27 &26.35 &18.80 &12.72 &9.47 &7.09 &25.37 &86.19 \\
mammal &28.40 &10.77 &23.45 &18.06 &9.81 &5.38 &3.39 &22.93 &86.44 \\
amphibian &27.74 &12.32 &23.95 &17.66 &11.34 &7.49 &5.60 &23.80 &86.26 \\
insect &28.35 &14.48 &24.97 &18.04 &12.10 &8.18 &5.70 &26.96 &86.41 \\
fish &31.67 &16.48 &27.53 &21.30 &14.62 &10.48 &8.01 &28.27 &86.51 \\
bird &30.72 &15.37 &26.90 &21.46 &14.90 &10.75 &8.55 &26.58 &85.94 \\
reptile &29.82 &15.41 &26.38 &19.09 &13.32 &9.51 &7.51 &28.60 &87.03 \\
celebrity &26.35 &12.96 &22.88 &17.52 &11.58 &8.30 &3.88 &19.43 &85.29 \\
instrument &30.32 &11.80 &24.59 &18.52 &10.52 &5.43 &3.47 &24.56 &87.06 \\
plant &31.37 &15.14 &27.78 &21.13 &13.15 &9.33 &7.68 &24.53 &85.95 \\
electronics &32.70 &15.47 &26.87 &20.04 &12.86 &8.19 &5.28 &28.86 &88.10 \\
tool &31.93 &14.68 &26.11 &19.34 &12.10 &8.34 &5.20 &28.73 &87.92 \\
transportation &29.12 &12.64 &23.87 &17.56 &10.42 &6.36 &3.94 &26.29 &87.70 \\
sport &26.15 &9.61 &20.87 &15.00 &7.88 &4.41 &2.41 &21.40 &86.25 \\
book &30.23 &13.97 &26.22 &20.23 &11.88 &7.61 &5.38 &23.80 &86.10 \\
household &32.91 &15.95 &27.39 &19.10 &12.13 &8.14 &5.81 &28.65 &88.22 \\
car &36.97 &17.09 &32.63 &27.25 &17.21 &7.72 &5.59 &28.52 &87.88 \\
\bottomrule
\end{tabular}

==> tables/openflamingo.tex <==
\begin{tabular}{lrrrrrrrrrr}\toprule
Method &ROUGE-1 &ROUGE-2 &ROUGE-L &BLEU-1 &BLEU-2 &BLEU-3 &BLEU-4 &METEOR &BertScore \\
\midrule
landmark &36.76 &20.26 &33.27 &17.13 &11.85 &8.75 &5.78 &21.41 &88.16 \\
painting &32.45 &16.50 &29.61 &17.14 &11.10 &7.44 &4.39 &19.48 &87.13 \\
sculpture &39.59 &23.26 &35.75 &19.58 &14.60 &11.10 &7.90 &23.65 &88.93 \\
food &34.71 &16.22 &30.87 &14.43 &9.46 &5.76 &3.57 &18.12 &88.32 \\
fruit &39.95 &24.19 &37.56 &24.42 &18.82 &15.24 &12.34 &27.77 &88.33 \\
vegetable &37.04 &20.46 &33.89 &19.19 &14.32 &11.13 &8.80 &23.37 &88.16 \\
mammal &32.98 &15.55 &29.29 &15.58 &10.03 &6.26 &4.51 &19.37 &87.91 \\
amphibian &32.65 &17.21 &29.85 &16.94 &12.35 &8.39 &6.39 &21.31 &87.82 \\
insect &35.15 &19.86 &32.07 &17.15 &12.76 &9.10 &6.66 &22.84 &87.30 \\
fish &39.67 &23.77 &36.58 &23.00 &17.64 &13.35 &10.54 &26.82 &88.51 \\
bird &37.13 &21.73 &34.11 &20.76 &16.04 &12.01 &9.80 &24.75 &88.10 \\
reptile &40.55 &23.87 &37.17 &22.36 &16.98 &12.24 &9.93 &27.02 &89.15 \\
celebrity &29.14 &16.16 &26.59 &16.04 &11.41 &8.38 &4.53 &18.20 &87.12 \\
instrument &34.62 &17.20 &30.80 &15.63 &10.75 &6.56 &4.60 &19.91 &88.58 \\
plant &36.56 &19.53 &33.79 &20.11 &14.49 &10.06 &8.11 &24.15 &86.76 \\
electronics &38.23 &22.76 &34.37 &17.61 &12.79 &8.92 &6.19 &23.22 &89.54 \\
tool &37.51 &19.77 &33.42 &18.60 &13.20 &9.52 &6.20 &24.37 &89.31 \\
transportation &35.35 &20.24 &32.54 &15.20 &11.43 &8.43 &6.08 &22.05 &89.10 \\
sport &28.29 &12.54 &24.46 &10.65 &6.28 &3.76 &1.61 &14.94 &87.61 \\
book &34.02 &18.94 &30.74 &19.10 &12.90 &9.04 &6.34 &21.82 &87.55 \\
household &39.44 &21.89 &34.67 &17.92 &13.05 &9.42 &6.82 &24.59 &89.60 \\
car &41.46 &23.40 &35.14 &24.80 &17.81 &9.53 &4.65 &26.40 &89.51 \\
\bottomrule
\end{tabular}
